Did You Really Just Have a Heart Attack? Towards Robust Detection of Personal Health Mentions in Social Media

Millions of users share their experiences on social media sites, such as Twitter, which in turn generate valuable data for public health monitoring, digital epidemiology, and other analyses of population health at global scale. The first, critical, task for these applications is classifying whether a personal health event was mentioned, which we call the (PHM) problem. This task is challenging for many reasons, including typically short length of social media posts, inventive spelling and lexicons, and figurative language, including hyperbole using diseases like "heart attack" or "cancer" for emphasis, and not as a health self-report. This problem is even more challenging for rarely reported, or frequent but ambiguously expressed conditions, such as "stroke". To address this problem, we propose a general, robust method for detecting PHMs in social media, which we call WESPAD, that combines lexical, syntactic, word embedding-based, and context-based features. WESPAD is able to generalize from few examples by automatically distorting the word embedding space to most effectively detect the true health mentions. Unlike previously proposed state-of-the-art supervised and deep-learning techniques, WESPAD requires relatively little training data, which makes it possible to adapt, with minimal effort, to each new disease and condition. We evaluate WESPAD on both an established publicly available Flu detection benchmark, and on a new dataset that we have constructed with mentions of multiple health conditions. Our experiments show that WESPAD outperforms the baselines and state-of-the-art methods, especially in cases when the number and proportion of true health mentions in the training data is small.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges
		

==> experiments-backup.tex <==
\section{Experimental Setup} \label{sec:exper-setup}
We begin this section by introducing the datasets that we used in the experiments. Then we discuss the baselines and the training setup.

\subsection{Datasets} \label{subsec:datasets}
We used the Flu dataset (\textit{awareness vs infection}) introduced in \cite{lamb2013separating}. Each tweet in the dataset is manually annotated as flu awareness (negative) or flu report (positive). At the crawling time, there were 2837 tweets available on Twitter, 1393 awareness tweets which account for 49\% of the dataset, and 1444 report tweets which account for 51\% of the dataset.

We also constructed a dataset consisting of 7192 English tweets across 6 diseases: Alzheimer, heart attack, Parkinson, cancer, depression, and stroke. We used the Twitter search API to retrieve the data in 3 different days. To retrieve the tweets, we used the disease names as keyword. After removing the re-tweets and replies the tweets were manually annotated. The labels are as follows:
\begin{itemize}[leftmargin=*]
\item \textit{self-mention}. The tweet contains a health mention to the Twitter account owner. e.g. \textit{"However, I worked hard and ran for Tokyo Mayer Election Campaign in January thru February, 2014, without publicizing the cancer."}
\item \textit{other-mention}. The tweet contains a health mention to someone other than the account owner. e.g. \textit{"Designer with Parkinson's couldn't work then engineer invents bracelet + changes her world"}
\item \textit{awareness}. The tweet contains the disease name, but does not mention a specific person. e.g. \textit{"A Month Before a Heart Attack, Your Body Will Warn You With These 8 Signals"}
\item \textit{non-health}. The tweet contains the disease name, but the tweet topic is not about health. \textit{"Now I can have cancer on my wall for all to see <3"}
\end{itemize}

\begin{table}
\caption{The distribution of tweets over topics and labels in the health dataset.} \label{tbl-health}
\begin{center}
\begin{tabular}{|p{0.6in} |p{0.3in} |p{0.4in} |p{0.4in} |p{0.45in} |p{0.4in} |}\hline
\textbf{Topic} & 
{\footnotesize \textbf{Tweet count}} & 
{\footnotesize \textit{self-mention}} & 
{\footnotesize \textit{other-mention}} & 
{\footnotesize \textit{awareness}} & 
{\footnotesize \textit{non-health}} \\ \hline
Alzheimer & 1256 & 1\% & 17\% & 80\% & 2\% \\ \hline 
heart attack & 1219 & 4\% & 9\% & 17\% & 70\% \\ \hline 
Parkinson & 1040 & 2\% & 9\% & 65\% & 24\% \\ \hline 
cancer & 1242 & 3\% & 18\% & 62\% & 17\% \\ \hline 
depression & 1213 & 37\% & 3\% & 49\% & 11\% \\ \hline 
stroke & 1222 & 3\% & 11\% & 29\% & 57\% \\ \hline 
\end{tabular}
\end{center}
\end{table}

In our experiments \textit{self-mention} and \textit{other-mention} labels are taken as positive set; and \textit{awareness} and \textit{non-health} labels are taken as negative set. To validate the labels, we engaged another annotator and randomly re-annotated 10\% of the tweets for each topic. Since we empirically observed that the probability of having a controversial positive label is more than having a controversial negative label, the 10\% subset was drawn from the positive set. The re-annotation showed 85\% agreement between the first and the second annotator, which is acceptable for a controversial topic like health report. Table \ref{tbl-health} summarizes the health dataset. One observation is that in each topic, a significant portion of the tweets are in \textit{non-health} category, which shows that people tend to use these words in other contexts too--which confirms the previous findings \cite{yin2015scalable}. The statistics also show that on average 19.5\% of the tweets in each topic are positive, which makes the classification task challenging. Having both a balanced dataset (the flu) and an imbalanced dataset (the health) helps us to evaluate our method and all the baselines in different environments.

To build the context features in the health dataset, we used the Twitter API to download the user timelines. We were unable to build the context features for the majority of the tweets in the flu dataset, since in many cases either the timeline was unaccessible or the access to the tweet was restricted. Therefore, we report the results for the flu dataset without incorporating the context features.

\subsection{Training setup} \label{subsec:train}
To parse and build the dependency tree for the tweet contents we used the parser introduced in \cite{kong2014dependency}. To extract the frequent subtrees, we used the approach proposed in \cite{matsumoto2005sentiment}, with minimum support 10 and minimum tree size 2. To estimate the value of the probabilistic function \textit{Pr} in our method (introduced in section \ref{subsec:new-mean}) we used the Mallet \cite{mccallum2002mallet} implementation of the multivariate logistic regression classifier with default settings. To partition the embedding space we used the ELKI \cite{schubert2015framework} implementation of the k-means clustering algorithm. We tried pretrained word2vec word embeddings \cite{mikolov2013distributed} (with 300 dimensions), and also pretrained Glove word embeddings \cite{pennington2014glove} (with 200 dimensions) in Twitter. In the next section we report the results achieved using word2vec word embeddings, however, the improvements are consistent if we use Glove word embeddings. To train the models (our model and the baselines) we used standard 10 fold cross validation in the flu dataset and in each topic of the health dataset--therefore, we split the data into 80\% training set, 10\% validation set, and 10\% test set; and iteratively replaced the folds. The results that we report in the next section are the average of the results in the test sets. To build the folds, we preserved the original distribution of the labels, and randomly assigned the tweets to each fold. Since the set of positive tweets is small, we kept the folding setting consistent for all the models, thus, they had identical set of tweets in the training, validation, and test sets. We used grid search to tune the model hyper-parameters to maximize F-measure in the positive set. Due to the small size of the positive sets in the health dataset, the accuracy of all the models was high (on average 90\%), therefore, in the next section we only report the F-measure, precision, and recall in the positive sets.

We used a logistic regression classifier trained over the final feature vectors to label the tweets \footnote{We also tried the SVM classifier with linear kernel, and initially achieved slightly better results. However, due to performance (speed) issues in the grid search, we replaced it with the logistic regression classifier.}. To tune the number of partitions \(K\) and \(K_2\) in the embedding space (introduced in sections \ref{subsec:par-emb} and \ref{subsec:we-mean}), we tried the value: \{3, 4, 5\}, and observed that their optimal values highly depend on the training data and were not fixed. To shrink the grid size in the tuning step we set \(\alpha\) to be equal to \(\alpha_2\) (introduced in sections \ref{subsec:new-mean} and \ref{subsec:we-mean}) and tried the values: \{0.05, 0.15, 0.3\}, and found them to be optimal at 0.05 in the flu dataset, and at 0.3 across all the topics in the health dataset. As baseline, we used the following models and implementations:

\begin{itemize}[leftmargin=*]
\item \textit{MaxEnt+lex}. We used a logistic regression classifier (a.k.a Maximum Entropy classifier) trained over unigrams and bigrams.
\item \textit{MaxEnt+cen}. We used a logistic regression classifier trained over the text centroid representation of the tweets in the embedding space.
\item \textit{MaxEnt+lex+emb}. We computed the text centroid representation of each tweet in the embedding space, and combined the resulting vector with the unigrams and bigrams of the tweet. Then a logistic regression classifier was trained over the final vectors.
\item \textit{MaxEnt+lex+cen}. We added two features PFlag and NFlag to the corresponding vector of unigrams and bigrams of each tweet. Then we used the output of \textit{MaxEnt+cen} to set the values of PFlag and NFlag. If the tweet was labeled positive we set PFlag, and if it was negative we set NFlag. Finally, a logistic regression classifier was trained over the resulting vectors. We used this model to evaluate our noise filtering method in section \ref{subsec:new-mean}.
\item \textit{Rules}. Experiments in \cite{lamb2013separating} suggest that manually extracted templates and features are effective in detecting flu reports. We implemented the top 6 set of features reported in \cite{lamb2013separating}, and trained a logistic regression classifier over the resulting vectors. This model was used only in the flu dataset.
\item \textit{CNN}. We used the convolutional neural network classifier introduced in \cite{kim2014convolutional}. We used the non-static variant, which can update the word vectors in the training. Using grid search we tuned the number of convolution feature maps from values: \{50, 100, 150\}, and observed that the number of features highly depends on the training data, and was not fixed. The rest of the hyperparameters were set to the suggested values \footnote{https://github.com/harvardnlp/sent-conv-torch}.
\item \textit{FastText}. We used the shallow neural network introduced in \cite{joulin2016bag}, known as FastText. This model represents the documents by taking average over the individual word vectors, and can also update the vectors during the training. To tune the model we tried values: \{0.05, 0.1, 0.25, 0.5\} for learning rate, and values: \{2, 4\} for window size. We observed that the value of learning rate was not fixed, neither in the flu dataset nor in the health dataset. The value of window size was optimal at 4 in the flu dataset, but was not fixed in the health dataset. The rest of the hyperparameters were set to the suggested values \cite{joulin2016bag}.
\item \textit{LSTM-GRNN}. We used the model proposed in \cite{tang2015document}, which is a two-step classifier. In the first step the model uses a long short-term memory neural network (LSTM) to produce the sentence representations, and in the second step, uses a gated recurrent neural network (GRNN) to encode the sentence relations in the document. To tune the model, we used values: \{0.03, 0.3, 0.5\} for learning rate, and observed that it is optimal at 0.3 in the flu dataset, but is not fixed in the health dataset. The rest of the hyperparameters were set to the suggested values \cite{tang2015document}.
\end{itemize}

We used the tweet dependency trees \cite{kong2014dependency} to detect sentence boundaries, which were needed in our model \MODEL to extract frequent subtrees, and also in \textit{LSTM-GRNN} model to produce the sentence representations. Although it is commonly known that deep neural network classifiers need a large training set to reach their best performance, we included these state-of-the-art baselines to investigate the models which are purely relying on word embeddings.

\section{Result and Discussion} \label{sec:results}
We report the results in section \ref{subsec:results}, and discuss different aspects of our model in section \ref{subsec:discuss}. We specifically try to investigate the importance of our features, and also explore the role of hyperparameters.


==> introduction-backup.tex <==
%\section{Introduction} 
%\label{sec:intro}

Among the social network applications, monitoring and analyzing the public health has been specifically focused due to the importance of the topic, and also the short comings of the traditional approaches. Public health tries to protect and promote the health of people and the environment that they live in. The traditional ways of public health surveillance include phone surveys, in-person interviews, and clinical reports. Phone surveys are biased \cite{blumberg2007coverage}, in-person interviews are expensive and slow \cite{iannacchione2011changing}, and clinical reports are limited and hard to establish. Therefore, social networks have obtained considerable attention, as an online and active environment, to monitor and analyze people's reports and reactions to the health related incidents. Detecting influenza epidemics \cite{aramaki2011twitter}, Dengue (a mosquito-borne infectious disease) surveillance \cite{gomide2011dengue}, tobacco use \cite{prier2011identifying}, drinking problems \cite{moreno2012associations}, public reactions to vaccination \cite{salathe2011assessing}, and wellness event detection \cite{akbari2016tweets} are a few studies of the ongoing research.

A crucial step in disease analysis and surveillance using social networks is to identify whether a specific user post is mentioning a person who is diagnosed with the disease or not. Any subsequent step and conclusion, whether it is epidemic detection (in case of mentioning an affected person in the post) or individual analysis (in case of reporting oneself health condition), highly depends on the quality of the initial identification. In this study, we try to identify the set of user posts which mention a person who is diagnosed with a specific disease, in the Twitter website. For instance, we desire to detect tweets like: \textit{"My grandpa has Alzheimer's \& he keeps singing songs about wanting to forget"} or \textit{"Yo Anti-Smoking group that advertises on twitch, I don't smoke. My mom died to lung cancer thanks to smoking for like 40 years. I get it."}, and also filter out the tweets like: \textit{"I almost had a heart attack when I found out they're doing a lettering workshop at @heathceramics in SF"} or \textit{"Dani seems like a cancer, spreads herself anywhere for attention!"}. Thus, given a tweet which contains a specific disease name, we try to identify whether the tweet mentions a person who is diagnosed with the disease or not. We assume it is a supervised learning process (there is a training set available for the disease), however, we also require that the solution must be general enough (topic independent) to be applied to other diseases too. We name this problem Personal Health Mention (\PROBLEM).

Due to the short length of user posts (140 characters) and also the diverse and informal language model of the users in Twitter, machine learning methods usually rely on extensive feature extraction to address sparsity in the feature space. In the contexts of company name detection \cite{spina2013discovering}, reputation measurement \citep{cha2010measuring}, sarcasm detection \cite{bamman2015contextualized,joshi2016word}, and also public health \cite{lamb2013separating,de2013predicting} methods are heavily dependent on augmenting user posts with complementary features collected from a variety of resources. In the health context, particularly, the training size is also affected by the frequency of the case reports, and therefore, it is highly imbalanced (our experiments show that on average 19\% of the tweets which contain a disease name, actually mention a person who is diagnosed with the disease). The direct implication of the imbalanced training data is that the classifier tends to have a high number of false negative cases (low recall), which may not be desirable in the applications such as disease surveillance or detecting epidemics. 

Although neural network classifiers have shown to be effective in the domains such as sentiment analysis, one particular drawback of the models is that it is not clear how to incorporate domain knowledge into the learning process. For instance, \cite{lamb2013separating} shows that the presence of specific phrases (word classes) are effective in flu detection, or \cite{de2013predicting} shows that the network properties can be used to detect user depression. These findings cannot be easily incorporated into a neural network classifier, therefore, exploring the approaches which utilize word embedding features in the classification process are desirable, and is the goal of this study. In this article we try to address the problems of sparsity and imbalanced training data through the generalization which is achieved using the word embedding space. In particular, we address the sparsity in the feature vectors through extracting additional features from the word embedding representation of the tweets. To address the imbalanced training data, we use the distribution of the training samples in the embedding space to acquire information about the unseen cases. One particular strength of our model is that it has the highest relative improvement when the ratio of the positive cases to the negative cases is low (between 0.1 to 0.3). These properties make our method particularly valuable for extending public health monitoring to a wider range of diseases and conditions. 

The main contributions of this paper are threefold:
\begin{itemize}[leftmargin=0.6cm]
\item We propose a novel, general approach to discover domain-specific signals in word embeddings to overcome the challenges inherent in the \PROBLEM problem. 
%This is the first study which tries to address the challenges in health case mention detection (specifically \PROBLEM problem) using the features extracted from the word embedding space.
\item We implement our approach as an effective PHM classification method, \MODEL (\textbf{W}ord \textbf{E}mbedding \textbf{S}pace \textbf{Pa}rtitioning and \textbf{D}istortion), which outperforms the state-of-the-art classifiers in almost all the disease cases.
\item To validate our approach, we have constructed a dataset consisting of 7,192 tweets across 6 topics: Alzheimer, heart attack, Parkinson, cancer, depression, and stroke. The tweets in the dataset are manually annotated, and used as the ground-truth in the experiments. We will make the dataset available to the research community to enable further progress on this problem.
\end{itemize}

Together, the approach, the method, and the experimental results and insights provide a significant advance in technology to enable online monitoring of health, by detecting personal health mentions in social media more accurately and with smaller amounts of  training data than previously possible. 
Next, we review the related work, which puts our contributions in context.


==> model-backup.tex <==
%\section{Model: \MODEL} 
%\label{sec:model}

This section introduces our method, \MODEL, for robust classificaiton of health mentiones in social media. We begin by summarizing the previously proposed lexical and syntactical features for health-related social media (primarily, Twitter) classification, which we implement as one of our baseline methods. We then introduce our new method, \MODEL, for learning topic-specific representation of the data based on the word embeddings (Sections~\ref{subsec:par-emb} and \ref{subsec:we-mean}). We conclude the section by describing how the \MODEL representation was operationalized as a health mention classifier, used in the experiments in the remainder of the paper.  

%We begin this section by reporting the lexical and syntactical features that we use in our model, and then continue the section by describing the word embedding based features that we propose to address the main challenges.

\subsection{Lexical and Syntactical Features} \label{subsec:lex-syn}
Studies on depression prediction \cite{de2013predicting}, flu detection \cite{lamb2013separating}, and tobacco use \cite{prier2011identifying} have shown that certain words and phrases are key indicators of the health reports, therefore, we use word unigrams and bigrams as features in the feature vectors. Additionally, to capture the long distance dependencies in the text, we use the approach proposed in \cite{matsumoto2005sentiment} to extract the syntactical dependencies in the tweets through detecting the frequent syntactical subtrees, and use them as features. We argue that, even with small amount of training data, the frequent subtrees can automatically detect a subset of the patterns which are usually designed manually for certain health cases (such as those of flu detection in \cite{lamb2013separating}). Although frequent item mining is expected to work best if enough data is available, by using the frequent subtrees, we at least expect to be able to extract the main frequent dependencies in the positive and negative classes. In the following subsections we discuss our new word embedding based features.

\subsection{Detecting noisy regions in embedding space} \label{subsec:new-mean}
Word embedding is a medium to map linguistic concepts to mathematical components (namely vectors). The motivation for using word embedding to address sparsity in our task is that it helps us to utilize partial matching in the model. Therefore, we can convert the sparse nominal space of the linguistic concepts into the measurable and aggregable space of the vectors. A common way to represent a short piece of text in the embedding space is to take the average of the constituent word vectors. Although this approach has some drawbacks, e.g. losing information about individual words, several studies have shown that if the text centroid is used in the proper way it can be effective \cite{kenter2015short,mihalcea2014simcompass,socher2013reasoning}. Here we analytically explore the ways that the centroid representation can be used to address the main challenges.

The main problem with representing a tweet using its centroid is that the centroid does not preserve information about the constituent words. This problem can be partially addressed through incorporating the information about the centroid as a complementary source of information and not as the final feature vector. Assuming that we had an approach to map the information about the centroid to a set of features, we could augment the set with the features discussed in section \ref{subsec:lex-syn}, and expect to have a better representation for the tweet. A straightforward way to use the information about the centroid along other features is to train a classifier over the tweet centroids in the training set and use the output of the classifier as a binary feature in the final feature vector. However, incorporating the class label, as is, would introduce the noise in the embedding space to the final classifier. We define the noisy regions in the embedding space to be the regions in which the classifier's precision is less than a certain threshold. Using tweet centroid as a complementary source of information enables us to filter out the regions which are noisy, and omit their contribution to the final feature vector. Detecting the regions which are not noisy also can help us to address the challenge of having imbalanced training set. These regions can be used in the model to safely predict the label of the instances which are not present in the training set. This can lead to a model which can potentially generalize better with small set of positive cases.

To detect the noisy regions in the embedding space we define probabilistic function \(Pr\) to be the probability of assigning the tweet centroid to the positive class. The values associated with \(Pr\) can be extracted from the training set using the logistic regression model. Given the function \(Pr\) and the associated values, the probability of assigning tweet \(t_i\) to the positive class would be \(Pr(t_i)\). Based on the definition, in the noisy regions the value of \(Pr\) is close to 0.5. Finally, we define binary features \(PFlag(t_i)\) and \(NFlag(t_i)\) for tweet \(t_i\) as follows:

\begin{displaymath}
	PFlag(t_i) = \begin{cases}
	1 & 0.5 + \alpha \leq Pr(t_i)\\
	0 & Otherwise
	\end{cases}
\end{displaymath}

\begin{displaymath}
	NFlag(t_i) = \begin{cases}
	1 & 0.5 - \alpha \geq Pr(t_i)\\
	0 & Otherwise
	\end{cases}
\end{displaymath}

in which \(\alpha\) is the threshold to detect the noisy regions, and can be tuned in the training phase. If tweet \(t_i\) is predicted to be positive and is not located in the noisy regions the value of \(PFlag(t_i)\) is set, and likewise, if it is predicted to be negative and is not located in the noisy regions the value of \(NFlag(t_i)\) is set.

\subsection{Partitioning the Word Embedding Space} 
\label{subsec:par-emb}

\(PFlag\) and \(NFlag\) can help us to capture the semantic similarity between the tweets which potentially belong to the same class. However, even though we try to reduce the degree of uncertainty in \(PFlag\) and \(NFlag\) through parameter \(\alpha\), they may still convey the noise in the embedding space to the final feature vectors. Additionally, the two features are not explicitly associated with the original lexical features, but are the result of a deduction about the tweet representation in the embedding space. Given that the feature vectors are sparse, \(PFlag\) and \(NFlag\) may effectively govern the whole computations, and potentially mislead the classifier. To reduce the effect of these features, and also to utilize the association between the lexical features and their representation in the embedding space, we constrain \(PFlag(t_i)\) and \(NFlag(t_i)\) to the region in the embedding space which \(t_i\) is located. Thus, we expect the two features also reflect the lexical similarity to some extent. The idea is illustrated in Figure \ref{fig:2d-space-combined}.

Figure \ref{fig:2d-space-combined} (a) shows a set of 1200 tweets projected to a two dimensional space using t-SNE \cite{maaten2008visualizing}. x-shaped data points denote the tweets which include a health mention. All the data points contain word \textit{heart attack}. Figure \ref{fig:2d-space-combined} (b) shows the same space with 3 hypothetical partitions, and a pair of features which is associated with each cluster. Given tweet \(t_i\) appearing in partition \(P_k\) feature \(PFlag_k(t_i)\) or \(NFlag_k(t_i)\) can be set. For instance, for the positive set of tweets which appear in partition P2, only the value of \(PFlag_2\) is set, and for the negative set of tweets which appear in partition P3, only the value of \(NFlag_3\) is set. This is essentially different from the idea of clustering the embedding space which has been tried before in different contexts \cite{mihalcea2014simcompass}. The partitions in our case are used to recover the lexical information, since the tweets which are close in the embedding space may also share lexical context. On the other hand, we don't expect to have pure partitions, and in fact, in \PROBLEM problem it is unlikely to have pure partitions. Because usually the training set is imbalanced, and the small set of positive cases is scattered in the space--due to sparsity. 

\begin{figure*}
\includegraphics[height=2in, width=6.6in]{2d-space-combined}
\caption{ (a) Set of 1200 tweet centroids that contain word \textit{heart attack}, projected to two dimensional space using t-SNE. (b) The same embedding space with 3 hypothetical clusters, and a pair of features associated with each cluster.} \label{fig:2d-space-combined}
\end{figure*}

The number of partitions (\(K\)) can be tuned experimentally in the training phase. In general, we expect large partitions improve recall and degrade precision. Because with larger partitions a higher number of tweets can be mapped to the same pair of \(PFlag\) and \(NFlag\), which can potentially increase the number of detected positive cases, and also increase the chance of mislabeling the tweets. 

\subsection{Distorting the Word Embedding Space}
\label{subsec:we-mean}

In section \ref{subsec:new-mean} we tried to partially address one of the drawbacks of using word embedding mean, that is the lose of information about the constituent words, through utilizing the mean along lexical features. However, this does not resolve the inherent problem of the mean. One approach to incorporate the information about individual terms is to integrate word importance into the averaging. For instance, to reduce the effect of less informative words on the mean, \cite{huang2012improving} suggests to use IDF-weighting to compute the weighted average of the word vectors in the sentence representation context. In classification context, we propose to use information gain \cite{mitchell1997machine} weighting to compute the mean vector to boost the impact of the words which are effective in the classification:

\begin{displaymath}
	\vec{M_t} = \frac{\sum_{i=0}^{n}IG_i \times \vec{W_i}}{\sum_{i=0}^{n}IG_i}.
\end{displaymath}

where $\vec{M_t}$ is the weighted mean vector for tweet \(t\), $\vec{W_i}$ is the vector representation of word $W_i$ in tweet \(t\), and $n$ is the length of the tweet. $IG_i$ is the information gain of word $W_i$ in the training set, and computed as follows:

\begin{displaymath}
	IG_i = Entr(D) - (\frac{|D_{w_i}|}{|D|} \times Entr(D_{w_i}) + \frac{|\overline{D_{w_i}}|}{|D|} \times Entr(\overline{D_{w_i}}))
\end{displaymath}

where \(D\) is the training set, \(Entr(D)\) is the entropy of \(D\) relative to our classification problem, \(|D|\) is the size of the training set, \(D_{w_i}\) is the subset of the training set for which \(W_i\) occurs, and \(\overline{D_{w_i}}\) is the subset of the training set for which \(W_i\) dost not occur. For the words which do not appear in the training set we estimate their information gain using the information gain of their closest word in the embedding space which also appear in the training set. Figure \ref{fig:2d-space-weighted} shows the same set of tweets which was used in Figure \ref{fig:2d-space-combined}, after applying IG-weighting. The projection shows that in some cases the transformation can successfully separate the less noisy regions.

\begin{figure}
\includegraphics[height=1.6in, width=3.3in]{2d-space-weighted}
\caption{The same set of tweet centroids reported in Figure \ref{fig:2d-space-combined}, after applying IG-weighting transformation.} \label{fig:2d-space-weighted}
\end{figure}

To use IG-weighting in our model we transform all the tweets using the information gain values extracted in the training set, and follow the model described in sections \ref{subsec:new-mean} and \ref{subsec:par-emb} to extract a set of features for each tweet. The values of parameter \(\alpha\) and the number of partitions \(K\), can be potentially different in the distorted embedding space, therefore, we call them \(\alpha_2\) and \(K_2\).

\subsection{Context in embedding space} \label{subsec:context}
Although, we do not restrict \PROBLEM problem to the cases which users report their own personal status (or even their relatives), it is still worthwhile to investigate the context in which users post the tweets. Previous studies in monitoring public health have shown that the user history is a good indicator of his current state, e.g. in depression detection \cite{de2013predicting}. We hypothesize that the profiles who post a tweet which include a personal health mention, might have already posted or will post a similar tweet. Although those tweets may not necessarily contain the disease keyword, they may be semantically or lexically similar to the current tweet. The requirements to support the hypothesis are precisely addressed by the model which we developed in section \ref{subsec:par-emb}. Therefore we use the model to extract a set of features based on the previous tweet, and also a second set of features based on the next tweet posted by the user.
